Self-Supervised Reinforcement Learning that Transfers using Random Features

Model-free reinforcement learning algorithms have exhibited great potential in solving single-task sequential decision-making problems with high-dimensional observations and long horizons, but are known to be hard to generalize across tasks. Model-based RL, on the other hand, learns task-agnostic models of the world that naturally enables transfer across different reward functions, but struggles to scale to complex environments due to the compounding error. To get the best of both worlds, we propose a self-supervised reinforcement learning method that enables the transfer of behaviors across tasks with different rewards, while circumventing the challenges of model-based RL. In particular, we show self-supervised pre-training of model-free reinforcement learning with a number of random features as rewards allows implicit modeling of long-horizon environment dynamics. Then, planning techniques like model-predictive control using these implicit models enable fast adaptation to problems with new reward functions. Our method is self-supervised in that it can be trained on offline datasets without reward labels, but can then be quickly deployed on new tasks. We validate that our proposed method enables transfer across tasks on a variety of manipulation and locomotion domains in simulation, opening the door to generalist decision-making agents.

==> rebuttal.tex <==

\newpage 
\section{General Response}

We are glad that all reviewers find our technical contribution significant and interesting, and we appreciate the concerns that the reviewers brought up. In response to these concerns, we have conducted a number of new experiments:  

- **Ability to deal with the infinite-horizon case:** To allow RaMP to scale up to infinite horizons, we introduce a modification that allows for on-policy estimation of infinite horizon returns during the learning of a new task. The key insight here is that we can use the linearly combined Q-function from RaMP to predict return over the first $H$ steps, following which we can use dynamic programming to estimate an estimate of the returns from $H$ to $\infty$ under the current policy. Using the Bellman update under deterministic transition dynamics, we can estimate the returns from $H$ to $\infty$, which can then be added to the estimated Q-function for the first $H$ steps as previously described in the paper. Importantly, even in this case with the return estimate from $H$ to $\infty$, the transfer performance from the first $H$ steps still does a bulk of the heavy lifting, since the tail of the returns from $H$ to $\infty$ is heavily discounted. For a detailed description of this technique and experimental results, please refer to Appendix E in the updated paper. We evaluate this method on four different environments, and find that it improves the performance on our longer-horizon environments but it doesn't significantly affect performance for manipulation tasks, likely because these tasks do not require infinite horizon reasoning. 

- **Ability to show continual improvement:** While we freeze the Q-basis networks at test time in our main experiments to demonstrate transfer behavior, we can in fact continuously improve both the Q-basis networks and the weight function by not just updating the weight function using least squares, but also allowing gradients to pass through into the Q-basis networks. In particular, we can finetune the Q-basis networks at test time by doing regression on the Monte-Carlo Q-function and allowing gradients to flow back into the Q-basis networks. We conduct finetuning experiments on Metaworld and D'Claw environments and show that it improves the performance of our method. For a detailed description of the method and the expertimental results, please refer to Appendix B.7 in the updated paper. In addition, our new modification in Appendix E that lets RaMP plan with infinite horizon $Q$-function will also allow continuous improvement as the value function estimation in it will continuously improve with more samples.

- **Better planning algorithm:** Our method is compatible with any planning method that generates sequences of actions and evaluates their returns using a model. To show the generality of the method, we provide additional results with the MPPI planner in Appendix B.6, which show that MPPI improves the performance of our method across a number of tasks. These results indicate that our method is fully general to different planning methods. 


These changes make the algorithm significantly more general, and we hope they address the concerns about the generality of the method and applicability across domains. We have also provided detailed responses to each reviewer's concern inline. 




\section{Reviewer 5Avm}
Thank you for your insights and comments. We have addressed your comments below. 

> *Q: Performance of each method on different areas of goals.* 

A: On inspection, we find that most of the model-free baseline comparisons - successor features, CQL do well in distribution of the training goals, but not on the out-of-distribution testing goals. RaMP on the other hand is able to retain in distribution performance while also extrapolating to OOD goals. Model-based RL methods like MBPO can work on OOD testing goals as well, but they struggle to perform well because of the challenges of compounding error and dimensionality, even in distribution. 
    
> *Q: Space complexity of RaMP and comparison with successor feature method.* 

A: The space complexity of RaMP is primarily determined  by the number of random features that are needed. As we describe in Corollary C.2, we require $K=\tilde\Omega({(1-\gamma)^{-2}\epsilon^{-2}})$ random features to achieve order-$\epsilon$ error between the estimated and true Q-function. As the required approximation error decreases, the space needed to store all the features grows sublinearly. Note that this result is for **any** given reward function (including the target one) under **any** policy $\pi$, but not tied to a specific one (under the realizability assumption of the reward function). 

On the other hand, the space complexity of the classical successor feature method is relatively fixed in the above sense: the dimension of the feature is fixed and does not change with the accuracy of approximating the **optimal** Q-function for the target task. However, the resulting guarantee is also more restricted: it is only for the optimal Q-function of the specific target reward, and also depends on the distance between the previously seen and the target reward functions. Hence, the two complexity are not necessarily comparable.  We have added this discussion to Appendix F. 

\section{Reviewer puvd}
Thank you for the helpful comments. We address your questions below.

> *Q: The finite horizon fixes the dependency of the Q function on the policy. However, it makes longer time horizon tasks intractable. This is a major weakness of the proposed approach.*

A: To allow RaMP to scale up to infinite horizons, we introduce a modification that allows for on-policy estimation of infinite horizon returns during learning of a new task. The key insight here is that we can use the linearly combined Q-function from RaMP to prediction return over the first $H$ steps, following which we can use dynamic programming to estimate an estimate of the returns from $H$ to $\infty$ under the current policy. With a simple Bellman update, we can estimate the returns from $H$ to $\infty$, which can then be added to the estimated Q-function for the first $H$ steps as currently described in the paper. Importantly, the transfer performance from the first $H$ steps does a bulk of the heavy lifting, since the tail of the returns from $H$ to $\infty$ is heavily discounted. For a detailed description of this technique and experimental results, please refer to Appendix E. We evaluate this method on four different environments, and find that it improves the performance on our longer-horizon environments but it doesn't improve performance for manipulation tasks, likely because these tasks do not require infinite horizon reasoning. 

> *Q: Trajectories are generated with random shooting. It's unclear how this would scale to continuous action spaces or longer horizon tasks.*

A: Our method is compatible with any planning method that generates sequences of actions and evaluates them using the model. To show the generality of the method, we provide additional results with MPPI planner in Appendix B.6, which show that MPPI improves the performance of our algorithm across a number of tasks. These results show that our method is fully general to different planning methods. To clarify, our experiments are on continuous action spaces *and* on long horizon tasks as shown in Section 4.3 and 4.4. But as shown in our new results, as the planning method is improved to MPPI this does improve performance. 

> *Q: How good are the reported results? That is, what would the score of a standard algorithm like PPO be in these cases (given enough training data).*

> *Q: What happens if training goes on for longer? MBPO is quickly improving in 5 of the 8 plots and it seems that if the plots were just a bit longer, the results would be much more positive for MBPO.*

A: Qualitatively, we find that the RaMP performance corresponds to solving the task (turning the faucet, successfully reaching the goal, moving the object with the claw). To provide a more fair baseline comparison we allowed MBPO to run for longer in the test domains and we find that it achieves somewhat better performance than RaMP given a much larger number of samples for some domains. We provide results with longer training in Fig $12$. This makes sense since MBPO is using a full dynamic programming update at test time while RaMP is only updating the reward weights using least squares. This suggests that the benefit of RaMP is largely in the low data regime for learning very quickly, as shown in Fig $3$. In fact, RaMP does not actually require active data collection in the test domain and can learn from just a small amount of provided data from the test domain. 

> *Q: RaMP seems to converge quickly and not improve anymore. This seems reasonable given that only the linear combination of Q-basis is learned. Can the learnt policy continue improving somehow?.*

A: Thanks for the great question! We can in fact continuously improve both the Q-basis networks and the weight function by not just updating the weight function using least squares but also allowing gradients to pass through into the Q-basis networks. At test time, we can finetune the Q-basis networks by doing regression on the Monte-Carlo Q-function and allowing gradients to flow back into the Q-basis networks. We provide finetuning results in Appendix B.7. and show that it improves the performance of our method. In addition, our new modification in Appendix E that lets RaMP plan with infinite horizon $Q$-function will also allow continuous improvement as the value function estimation in it will continuously improve with more samples.


> *Q: It's unclear that any reasonable number of random features will make the approach work in high-dimensional spaces. The only experiments in this setup are in the Appendix and are not very convincing. Why do you not make a comparison to MBPO, SF or other offline RL approaches in this setup?*

A: To the best of our knowledge, Dreamer is the state-of-the-art in image-based domains. MBPO performs worse than Dreamer with pixel observations because it does not handle non-Markovian observations, and SF does not scale to high-dimensional observations. We have included comparisons to Dreamer in Appendix B.4 which show that RaMP is competitive on several image based domains. 	

We hope our responses have addressed your comments. Feel free to let us know if you have any other questions. We are more than happy to address them. 

\section{Reviewer xLea}

Thank you for your careful reading and constructive comments. We address your questions below.

> *Q: Explanations about the theory part.*

A: For Theorem 3.1, due to space limitation, we only provided an “informal” statement in the main text, and deferred the detailed version in Appendix C. In the formal version of the statement in Theorem C.1, we **did** state the distribution of the random features (as well as the data). In particular, in Theorem C.1, the features $\phi(s,a;\theta)$ are parameterized by $\theta$, and $\theta$ is randomly drawn from distribution $p$. Note that the generalization error is not necessarily going to zero, as the right-hand side of the theorem contains some “inherent” error term $\inf_{f\in\mathcal{H}}\mathcal{E}(f)$, which is related to both the feature function $\phi$, as well as the parameter distribution $p$. In other words, the effect of the feature distributions is expressed in the form of this $\inf_{f\in\mathcal{H}}\mathcal{E}(f)$. A bad distribution (and feature function) would lead to a large error term; and in the “realizable” case (as some statistical learning theory result assumes), this inherent error would become zero, and the generalization error will **only decrease** as the number of samples $n$ increases. We wrote the result in a fairly general way to accommodate both cases. Regarding the result in Rudi and Rosaco (2017), we wrote the function class $\mathcal{H}$ in a slightly different but equivalent way as the RKHS one stated in the original theorem, for ease of presentation. Please see the discussion in Rudi and Rosaco (2017) around Eq. (10) for more discussions.

For Theorem 3.2, we first note that the whole point of this result is that the policy class doing policy improvement over, $\Pi$, is a **subclass/subset** of all the Markov stationary policies. We care about a subset of policies since this $\Pi$ usually corresponds to the set of policies that have been computed so far, and we would like to see that if we improve over all the policies in this set, the resulting policy's value function is not worse. See [1] for more discussions about this idea of "general policy improvement". When $\Pi$ becomes the whole policy set, yes, the reviewer is correct that "it cannot be improved upon" and our result (and even the one-step generalized policy improvement result in [1]) becomes vacuous. However, this is not the most interesting case people care about. Moreover, sorry for the confusion, for this part, we indeed meant "deterministic transitions", since this part was meant to justify our experiments, and all of them are done in this deterministic setting. We have now included this assumption formally. Finally, yes, there is some misunderstanding: the first inequality cannot be an equation, since the left-hand side is the value "under this policy $\pi_H$", while the right-hand side is the (multi-step) greedy of a "maximum" of multiple Q-functions under different policies, which might not correspond to the Q-function of **any** policy. In other words, the first inequality is **not** a Bellman equation.

> *Q: Number of steps is low: how do we perform with more number of steps, especially when compared with MBPO?*

A: We emphasize the transfer ability of our method in the low-data regime. We show that our method converges to the same performance as MBPO with enough steps and some additional modifications for online training. We also include additional comparisons with longer training in Appendix E, showing the improvements in the low data regime. 

> *Q: Only maximize reward only for the duration of the action sequence itself.*

A: While prior work on model-based planning uses a similar setting (PETS, Planet, LatCo), we also introduce modifications that allow for infinite horizon reasoning. To allow RaMP to scale up to infinite horizons, we introduce a modification that allows for on-policy estimation of infinite horizon returns during learning of a new task. The key insight here is that we can use the linearly combined Q-function from RaMP to prediction return over the first $H$ steps, following which we can use dynamic programming to estimate an estimate of the returns from $H$ to $\infty$ under the current policy. With a simple Bellman update, we can estimate the returns from $H$ to $\infty$, which can then be added to the estimated Q-function for the first $H$ steps as currently described in the paper. Importantly, the transfer performance from the first $H$ steps does a bulk of the heavy lifting, since the tail of the returns from $H$ to $\infty$ is heavily discounted. For a detailed description of this technique and experimental results, please refer to Appendix E. We evaluate this method on four different environments, and find that it improves the performance on our longer-horizon environments but it doesn't significantly affect performance for manipulation tasks, likely because these tasks do not require infinite horizon reasoning. 

> *Q: How RaMP learns the reward function in a new environment.*

A: We perform online least-squares regression by combining the reward basis to fit the reward from online experience.

> *Q: Why RaMP's performance even changes over time.*

A:  RaMP estimates the reward weights using online least squares. The least squares estimates improves as we get more data in the new task, leading to improved performance over time. We additionally introduce a new method for also improving the Q-basis functions as described in Appendix B.7. 

> *Q: What does "zero-shot" mean in Sec. 2.1*

A: zero-shot means we don't need online interactions with the new environment to get a policy. If some offline data in the form of $(s,a,r)$ tuples are given, we can fit our $\omega$ with linear regression and use this regressed $\omega$ with $Q$-basis with MPC planner to get a valid policy, without online interaction with the environment.

> *Q: Why jumping and running backward have drastically different objectives.*

A: Our offline rollout are collected via epsilon exploration using policies that runs forward at varying speeds. In a typical goal-conditioned setting, we input desired horizontal speed as goals. Jumping doesn't fits into this goal conditioned setting since it not only needs the robot to stay at origin but also jump. Running backward is also very different here because it's not only out of distribution but also requires the robot to run at the opposite direction which its mechanical structure isn't designed to do. For example, since humans have knees bending to the front, running forward is very different from running backward. 

> *Q: Reproducibility is not great.*

A: We will release the source code for our method upon acceptance, and all results can be reproduced. 

We hope our responses have addressed your comments. Feel free to let us know if you have any other questions. We are more than happy to address them.


[1] Barreto, André, Will Dabney, Rémi Munos, Jonathan J. Hunt, Tom Schaul, Hado P. van Hasselt, and David Silver. "Successor features for transfer in reinforcement learning." Advances in Neural Information Processing Systems 30 (2017).

 
\section{Reviewer R3oi}  

Thank you for your careful reading and constructive comments. We address your questions below.

> *Q: For large horizon $H$.*

A: In most of the experiments we ran, using a horizon of $H=10$ or $H=32$ was able to achieve good performance. Note that, this $H$ is **not** the horizon of the problem, but the planning horizon of the open-loop sequence. As one of the reviewers suggested, we have introduced a way to incorporate the infinite-horizon reward-to-go from horizon $H$, i.e., we can now handle larger or even infinite-horizon setting. We presented the new experimental results in Appendix E.2, and the statement of the approach in Appendix E.1 in our updated paper. In brief, this works by doing a Bellman update to learn the discounted value function from $H$ to $\infty$ on-policy which is added to the sum of rewards for the first $H$ steps. 


> *Q: Comment on implicit assumptions.*
A: We are interested in handling deterministic transition systems (and pointed it out explicitly now in our theory part). The open loop trajectory sequences make the method incompatible with stochastic dynamics. 

> *Q: Other optimization methods?*

A: We provide additional results with an MPPI planner in Appendix B.6 and show that it leads to improvements across multiple tasks. Instead of simply doing random shooting, we iteratively reweight the action sampling distribution using MPPI and find that on Metaworld and D'Claw environment this leads to both faster learning and higher asymptotic performance than random shooting. We emphasize that the main contribution of our paper is a method for fast adaptation, and it is compatible with any planning algorithm that evaluates open-loop action sequences.

We hope our responses have addressed your comments. Feel free to let us know if you have any other questions. We are more than happy to address them.



